Neural Multi-Quantile Forecasting for Optimal Inventory Management

In this work we propose the use of quantile regression and dilated recurrent neural networks with temporal scaling (MQ-DRNN-s) and apply it to the inventory management task. This model showed a better performance of up to 3.2\% over a statistical benchmark (the quantile autoregressive model with exogenous variables, QAR-X), being better than the MQ-DRNN without temporal scaling by 6\%. The above on a set of 10,000 time series of sales of El Globo over a 53-week horizon using rolling windows of 7-day ahead each week.

==> iclr/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/section3_orax_pipeline_dep.tex <==
\subsection{Forecasting Pipeline}

\textcolor{green}{Federico Descripción de Pipeline Actual}

Steps:

Sección modelos a ensamblar.



\begin{enumerate}
    \item \textbf{Data storage}
    \begin{itemize}
        \item GLB dataset:
        \item BRC dataset:
    \end{itemize}
    \item \textbf{Featurization}
    \begin{itemize}
        \item Univariate models: trained using Hyndman's forecast package.
        \begin{itemize}
            \item AutoARIMA
            \item ETS
            \item Theta
            \item Naive
            \item Naive2
            \item SeasonalNaive
            \item TBATS
            \item NNETAR
            \item STLM
            \item RandomWalk with Drift
        \end{itemize}
        \item Features:
    \end{itemize}
    \item \textbf{Train and set sets}
    \begin{itemize}
        \item 
    \end{itemize}
    \item \textbf{FFORMA forecasts}
    \begin{itemize}
        \item 
    \end{itemize}
\end{enumerate}

- Poner cita.
- Ajustar tamaño para notas.
- Caption.

\begin{table}[htpb]
\tiny
\centering
 \begin{tabular}{p{0.2\linewidth} | p{0.8\linewidth}}
        \toprule
                  Feature & Meaning \\
        \midrule
              unitroot\_pp & The statistic for the $Z-\alpha$ version of Phillips and Perron unit root test with constant trend and lag 1.\\
            unitroot\_kpss & The statistic for the Kwiatkowski et al. unit root test with linear trend and lag 1.         \\
                 hw\_alpha & $\alpha$  parameter of an $ets(A,A,A)$ model fitted on the series.\\
                  hw\_beta & $\beta$ parameter of an $ets(A,A,A)$ model fitted on the series.         \\
                 hw\_gamma & $\gamma$  parameter of an $ets(A,A,A)$ model fitted on the series.        \\
                stability & The variance of the means based on a division of the series in non-overlapping portions. The size of the portions is the frequency of the series, or 10 if the series has frequency 1.\\
                    trend & In a STL decomposition of the series with $r_t$ the remainder series and $z_t$ the deseasonalized series: $max(0,1 - \Var(r_t)/\Var(z_t))$.        \\
                    spike & In a STL decomposition of the series with $r_t$ the remainder series, the variance of the leave one out variances of $r_t$.        \\
                linearity & In a STL decomposition of the series with $T_t$ the trend component, a quadratic model depending on time is fitted: $T_t=\beta_0+\beta_{1} t+\beta_2 t^2+\varepsilon_t$. Linearity is $\beta_1$.        \\
                curvature & In a STL decomposition of the series with $T_t$ the trend component, a quadratic model depending on time is fitted: $T_t=\beta_0+\beta_1 t + \beta_2t^2 + \varepsilon_t$. Curvature is $\beta_2$.         \\
                   e\_acf1 & The first autocorrelation coefficient of the remainder series in an STL decomposition of the series.         \\
                  e\_acf10 & The sum of the first 10 squared autocorrelation coefficients of the remainder series in an STL decomposition of the series.         \\
        seasonal\_strength &  In a STL decomposition of the series with $r_t$ the remainder series and $x_t$ the detrended series: $max(0, 1 - \Var(r_t)/\Var(x_t))$. \\
                     peak & The location of the peak (maximum value) in the seasonal component of and STL decomposition of the series.        \\
                   trough & The location of the trough (minimum value) in the seasonal component of and STL decomposition of the series.        \\
                  x\_pacf5 & The sum of squared first 5 partial autocorrelation coefficients of the series.         \\
             diff1x\_pacf5 & The sum of squared first 5 partial autocorrelation coefficients of the first differenced series.        \\
             diff2x\_pacf5 & The sum of squared first 5 partial autocorrelation coefficients of the twice differenced series.        \\
                seas\_pacf & The partial autocorrelation coefficient at the first seasonal lag. 0 if the series is non seasonal.         \\
             nonlinearity & A nonlinearity statistic based on Terasvirta’s nonlinearity test of a time series.        \\
                lumpiness & The variance of the variances based on a division of the series in non-overlapping portions. The size of the portions if the frequency of the series, or 10 is the series has frequency 1.        \\
                    alpha & The smoothing parameter for the level in a $ets(A,A,N)$ model fitted to the series.        \\
                     beta & The smoothing parameter for the trend in a $ets(A,A,N)$ model fitted to de series.        \\
                 arch\_r2 &  After the series is pre-whitened using an $AR$ model and squared, the $R^2$ value of an $AR$ model applied to it.        \\
                garch\_r2 &  After the series is pre-whitened using an $AR$ model, a $GARCH(1,1)$ model is fitted to it and the residuals are calculated. The sum of squares of the first 12 autocorrelations of the squared residuals.        \\
                  arch\_acf & After the series is pre-whitened using an $AR$ model and squared, the sum of squares of the first 12 autocorrelations. \\
                 garch\_acf & After the series is pre-whitened using an AR model, a $GARCH(1,1)$ model is fitted to it and the residuals are calculated. The sum of squares of the first 12 autocorrelations of the squared residuals.        \\
               flat\_spots & The number of flat spots in the series, calculated by discretizing the series into 10 equal sized intervals and counting the maximung run length within any single interval.         \\
          crossing\_points & The number of times the time series crosses the median. \\
                  arch\_lm & A statistic based on the Lagrange Multiplier test of Engle (1982) for autoregressive conditional heteroscedasticity.The $R^2$ of an autoregressive model of 12 lags applied to $x^2$ after the its mean has been subtracted.        \\
                   x\_acf1 & The first autocorrelation coefficient of the series.         \\
                  x\_acf10 & The sum of the squared first ten autocorrelation coefficients of the series. \\
               diff1\_acf1 & The first autocorrelation coefficient of the first differenced series. \\
              diff1\_acf10 & The sum of the squared first ten autocorrelation coefficients of the first differenced series. \\
               diff2\_acf1 & The first autocorelation coefficient of the twice-differenced series.\\
              diff2\_acf10 & The sum of squared fist ten autocorrelation coefficients of the original series.\\
                seas\_acf1 &The autocorrelation coefficient at the first seasonal lag.          \\
        \bottomrule
\end{tabular}
\caption{Features used by FFORMA.}
\label{table:hyndman_features}
\end{table}   

\begin{itemize}
    \item Data storage.
    \item Split validation and train sets. Validation size is equal to forecasting horizon.
    \item Train and predict each model for each time series on validation set and get the best set of parameters for each model.
    \item Featurize validation and train sets.
    \item Train fforma on validation set to get the best set of hyperparamteters.
    \item Train and predict the forecasting horizon using each model for each time series.
    \item Ensemble results using fforma.
\end{itemize}

Featurization:
- Models.
- Tsfeature.

No rollear xgboost.
- Usar hiperparámetros de Hyndman para todo el año (esto reduce el costo).
- Buscar hiperparámetros con un año entero de validación.

Notas:
- Más preciso en data wrangling, storage, featurization.
- Sub-bullets.




esta información la va a tener Federico vas a tener que pingearlo hasta que te de su pdf del Orax pipeline y el pipeline anterior.

pensar los limites, porqué sirve lo que estamos haciendo?
a quién sirve lo que estamos haciendo?

\begin{itemize}
    \item por qué estimar con promedios moviles
    \item por qué estimar con medias auto regresivas
    \item por qué estimar con modelos Naive
\end{itemize}

potencialmente provoca problemas al modelo de subestimación de predicciones
Qué implicaciones tiene para las personas que ejecutan las predicciones y porqué al final las predicciones siempre se inflan con heurísticas mafufas como multiplicar por porcentajes raros.

\textcolor{green}{Federico Mejorar/parafrasear esta gráfica usando keynote o ppt y exportar a pdf}

\begin{figure}[htpb]
\begin{center}
\includegraphics[scale=0.25]{images/pipeline_placeholder.jpeg}
\end{center}
\caption{Orax Pipeline}
\label{fig:pipeline}
\end{figure}

\subsection{Datasets}

\textcolor{green}{Descripción Federico de datos},
\begin{itemize}
    \item datos panel de demanda en unidades para productos para Globo y Barcel a nivel nacional
    \item Filtro de tiempo
    \item Filtro de velocidad (demanda mínima)
\end{itemize}



Two sets of data, D1 and D2, obtained from the daily operation of two of the largest companies in Mexico in the area of retail sales, were chosen to evaluate the models. Both sets consist of 10,000 time series with daily periodicity. The first set, denoted by D1, contains observations from 2018-05-24 and until 2020-02-29; while the second set, denoted by D2, contains observations from 2018-01-01 and until 2020-02-29. Due to the characteristics of the business, the missing values were replaced with 0. In both cases, the time series were chosen to have the highest number of sales.

\subsection{Dataset Processing}

\textcolor{green}{Federico Escribir Tabla descriptiva de variables},

Tabla con descripción de las variables que usamos, podemos hacerla con formato X, S, Y
recomiendo hacer la tabla antes en excel que quede bonita y que pasemos después a latex con la pagina de excel to latex.

Probablemente podemos describir un poco el proceso de creación de las variables.

\begin{itemize}
    \item nombre de variable
    \item descripción
\end{itemize}

==> sections/section5_discussion.tex <==
This Section presents four ideas to be explored following the research conducted in this work. The first extension consists of comparing the preprocessing proposed in the MQ-DRNN-s model for parametric models. The second and third extensions concern the adaptation of this idea to different time series problems. Finally, the fourth proposal is based on considering other time scaling functions.

\textcolor{red}{se sugiere eliminar, considerar}

\section{Parametric forecast}

An extension of the work presented here is the use of temporal scaling for parametric forecasting. That is, seeking to model the parameters of a known distribution with machine learning models \citep{flunkert2017deepAR,mukherjee2018armdn}. In particular, a specific research direction is to use count distributions such as Poisson, negative binomial and mixtures such as Zero-Inflated Poisson (ZIP) \citep{zipregression}, a mixture of a Poisson distribution and a degenerated distribution at zero, as the data used in this paper is sparse.

\section{Hierarchical forecasting}

Hierarchical forecasting seeks to generate forecasts for different levels of aggregation of the time series \citep{hyndman_book}. For example, in addition to the sales center, at the state or regional level. An extension of this work is to adapt the model to generate hierarchical multi-quantile forecasts to obtain different scenarios for each level of aggregation.

\section{Meta Learning}
Meta-learning for time series is based on the training of different models to ensemble them automatically following a criterion (FFORMA; \cite{MONTEROMANSO202086}). Generally, this ensemble is built using machine learning models. In this sense, meta-learning automates the forecaster's work in terms of model selection. A potential extension is the investigation of quantile ensembles which involves a theoretical development as the arithmetic aggregation of quantiles is not well defined.

\section{Other level models}

In the MQ-DRNN-s model, the median of the time series is used as preprocessing function. A natural question is whether different scaling functions improve the performance of the model. This idea is a direct extension of the work, mainly using specific models for modeling sparse time series such as the Croston's model \citep{croston}.
